Rate of convergence of attractors for semilinear singularly perturbed problems: parabolic equations with large diffusion

We exhibit a singularly perturbed parabolic problems for which the asymptotic behavior can be described by an one-dimensional ordinary differential equation. We estimate the continuity of attractors in the Hausdorff metric by rate of convergence of resolvent operator.

==> References.tex <==
% This file was created with JabRef 2.10b2.
% Encoding: UTF-8


@Book{A.N.Carvalho2010a,
  Title                    = {Attractors for infinite-dimensional non-autonomous dynamical systems},
  Author                   = {A. N. Carvalho, J.A. Langa, J.C. Robinson,},
  Editor                   = {Springer},
  Year                     = {2010},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{flank,
  Title                    = {Rate of convergence of Attractors for some sinsingular perturbed parabolic problems},
  Author                   = {J. M. Arrieta and F.D.M. Bezerra and A. N. Carvalho},
  Journal                  = {Top. Methdos Nonlinear Anal},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{J.M.Arrieta2000,
  Title                    = {Attractors for parabolic pro\-blems with nonlinear boundary bondition. Uniform bounds},
  Author                   = {J. M. Arrieta and A. N. Carvalho and A. Rodr{\'\i}guez-Bernal},
  Journal                  = {Commun. in partial differential equations},
  Year                     = {2000},
  Pages                    = {1-37},
  Volume                   = {25},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{J.M.Arrieta2000a,
  Title                    = {Upper semicontinuity for attractors of parabolic problems with localized large diffusion and nonlinear boundary conditions},
  Author                   = {J. M. Arrieta and A. N. Carvalho and A. Rodr{\'\i}guez-Bernal},
  Journal                  = {Journal of Differential Equations},
  Year                     = {2000},
  Pages                    = {33-59},
  Volume                   = {168},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{J.M.Arrieta1999,
  Title                    = {Parabolic problems with nonlinear boundary conditions and critical nonlinearities},
  Author                   = {J. M. Arrieta and A. N. Carvalho and A. Rodr{\'\i}guez-Bernal},
  Journal                  = {Journal of Differential Equations},
  Year                     = {1999},
  Pages                    = {376-406},
  Volume                   = {156},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{Carbone2006,
  Title                    = {Continuity of the attractors in a singular problem arising in composite materials},
  Author                   = {V. L. Carbone and J. G. Ruas-Filho},
  Journal                  = {Nonlinear Anal},
  Year                     = {2006},
  Pages                    = {1285-1305},
  Volume                   = {65},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{Carvalho2010,
  Title                    = {Equi-exponential attraction and rate of convergence of attractors for singularly pertubed evolution equations},
  Author                   = {A.N. Carvalho and J.W. Cholewa and T.Dlotko},
  Journal                  = {Cadernos de matemática},
  Year                     = {2010},
  Pages                    = {111-151},
  Volume                   = {11},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{E.R.Aragao-Costa2011,
  Title                    = {Stability of gradient semigroups under perturbations},
  Author                   = {E.R. Aragão-Costa, T. Caraballo, A. N. Carvalho, J.A.Langa},
  Journal                  = {Nonlinearity},
  Year                     = {2011},
  Volume                   = {24},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Book{Henry1980a,
  Title                    = {Geometric theory of semilinear parabolic equations},
  Author                   = {Dan Henry},
  Editor                   = {Springer-Verlag},
  Publisher                = {Lecture Notes in Mathe\-matics},
  Year                     = {1980},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@PhdThesis{Pires2013,
  Title                    = {Taxa de atração para equações com difusão grande localizada},
  Author                   = {Leonardo Pires},
  School                   = {UfSCar},
  Year                     = {2013},
  Type                     = {Dissetação de mestrado},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}

@Article{Santamaria2014,
  Title                    = {Estimates on the distance of inertial manifolds},
  Author                   = {E. Santamaria and J. M. Arrieta},
  Journal                  = {Discrete and continuous dinamical systems},
  Year                     = {2014},
  Number                   = {10},
  Pages                    = {3921-3944},
  Volume                   = {34},

  Owner                    = {lplplp},
  Timestamp                = {2014.10.20}
}


